Carbon-Efficient Software Design and Development: A Systematic Literature Review

The ICT sector, responsible for 2% of global carbon emissions, is under scrutiny calling for methodologies and tools to design and develop software in an environmentally sustainable-by-design manner. However, the software engineering solutions for designing and developing carbon-efficient software are currently scattered over multiple different pieces of literature, which makes it difficult to consult the body of knowledge on the topic. In this article, we precisely conduct a systematic literature review on state-of-the-art proposals for designing and developing carbon-efficient software. We identify and analyse 65 primary studies by classifying them through a taxonomy aimed at answering the 5W1H questions of carbon-efficient software design and development. We first provide a reasoned overview and discussion of the existing guidelines, reference models, measurement solutions and techniques for measuring, reducing, or minimising the carbon footprint of software. Ultimately, we identify open challenges and research gaps, offering insights for future work in this field.

==> tab/selected-studies.tex <==
\scriptsize
    \resizebox{.99\textwidth}{!}{
    \begin{tabular}{clc}
        \hline
        \rowcolor{headergray}
        \textbf{Ref.} & \textbf{Author(s). \textit{Title}} & \textbf{Year}
        \\
        \hline
        \cite{16_Ahmed2020_codingCloud} & Ahmed.  \textit{Environmental sustainability coding techniques for cloud computing} & 2020 \\ 
        \rowcolor{rowgray}
        \cite{31_Alofi2023_Self-Optimizing} & Alofi et al. \textit{Self-optimizing the environmental sustainability of blockchain-based systems} & 2023 \\ 
        \cite{30_Alofi2022_OptimizingConsensus} & Alofi et al. \textit{Optimizing the energy consumption of blockchain-based systems using evolutionary algorithms: a new problem formulation} & 2022 \\ 
        \rowcolor{rowgray}
        \cite{18_Atkinson2014_GreenSpecifications} & Atkinson et al. \textit{Facilitating greener IT through green specifications} & 2014 \\ 
        \cite{50_Becker2016_Requirements} & Becker et al. \textit{Requirements: the key to sustainability} & 2016 \\ 
        \rowcolor{rowgray}
        \cite{21_Beghoura2014_GreenEvaluation} & Beghoura et al. \textit{Green application awareness: nonlinear energy consumption model for green evaluation} & 2014 \\ 
        \cite{17_Brownlee2021_AccuracyEnergyML} & Brownleee et al. \textit{Exploring the accuracy-energy trade-off in machine learning} & 2021 \\ 
        \rowcolor{rowgray}
        \cite{01_Chauhan2013_GreenSDLCCloud} & Chauan and Saxena. \textit{A green software development life cycle for cloud computing} & 2013 \\
        \cite{36_Fernandez2018_GreenDesign} & Condori-Fernàndez and Lago. \textit{The influence of green strategies design onyo quality requirement prioritization} & 2018 \\ 
        \rowcolor{rowgray}
        \cite{24_Dick2013_GSE-Agile} & Dick et al. \textit{Green software engineering with agile methods} & 2013 \\ 
        \cite{48_Dick2010_GreenSustainableSoftware} & Dick et al. \textit{A model and selected instances of green and sustainable software} & 2010 \\ 
        \rowcolor{rowgray}
        \cite{32_Fakhar2012_GreenComputing} & Fakhar et al. \textit{Software level green computing for large scale systems} & 2012 \\ 
        \cite{52_Fu2021_ComputerVision} & Fu et al. \textit{Reconsidering CO2 emissions from computer vision} & 2021 \\ 
        \rowcolor{rowgray}
        \cite{51_LeGoaer2021_greenCode} & Le Goaër. \textit{Enforcing green code with Android lint} & 2021 \\ 
        \cite{13_LeGoaer2023_ecoCodeProject} & Le Goaër. \textit{Decarbonizinf software with free and open-source software: the ecoCode project} & 2023 \\ 
        \rowcolor{rowgray}
        \cite{49_LeGoaer2023_ecoCode} & Le Goaër. \textit{ecoCode: a SonarQube plugin to remove energy smells from Android projects} & 2023 \\ 
        \cite{15_Heithoff2023_DigitalTwins} & Heithoff et al. \textit{Digital twins for sustainable software systems} & 2023 \\ 
        \rowcolor{rowgray}
        \cite{39_Hoesch-Klohe2010_GreenBPM} & Hoesch-Klohe et al. \textit{Towards green business process management} & 2010 \\ 
        \cite{34_Ibrahim2021_GSDProcessModel} & Ibrahim et al. \textit{The development of green software process model: a qualitative design and pilot study} & 2021 \\ 
        \rowcolor{rowgray}
        \cite{25_Ibrahim2022_GreenFactors} & Ibrahim et al. \textit{Green software process factors: a qualitative study} & 2022 \\ 
        \cite{07_Jayanthi20211_OrganizationalStructure} & Jayanthi et al. \textit{An organizational structure for sustainable software development} & 2021 \\ 
        \rowcolor{rowgray}
        \cite{26_Jebraeil2017_gUML} & Jebraeil et al. \textit{gUML: Reasoning about energy at design time by extending UML deployment diagrams with data centre contextual information} & 2017 \\ 
        \cite{46_Johann2011_IntegratedApproach} & Johann et al. \textit{Sustainable development, sustainable software, and sustainable software engineering: an integrated approach} & 2011 \\ 
        \rowcolor{rowgray}
        \cite{03_Karunakaran2013_PetriNet} & Karunakaran and Rao. \textit{A petri net simulation of software development lifecycle towards green IT} & 2013 \\ 
        \cite{54_Kern2013_GreenSA} & Kern et al. \textit{Green software and green software engineering -- definitions, measurements, and quality aspects} & 2013 \\ 
        \rowcolor{rowgray}
        \cite{61_Kern2015_ICTCO2footprint} & Kern et al. \textit{Impacts of software and its engineering on the carbon footprint of ICT} & 2015 \\ 
        \cite{33_Kern2018_AssessCriteria} & Kern et al. \textit{Sustainable software products -- Towards assessment criteria for resource and energy efficiency} & 2018 \\ 
        \rowcolor{rowgray}
        \cite{64_Kharchenko2013_VonNeumannParadigm} & Kharchenko and Gorbenko. \textit{Evolution of von Neumann's paradigm: dependable and green computing} & 2013 \\ 
        \cite{62_Kipp2011_GreenMetrics} & Kipp et al. \textit{Green metrics for energy-aware IT systems} & 2011 \\ 
        \rowcolor{rowgray}
        \cite{28_Kipp2012_GreenIndicators} & Kipp et al. \textit{Layered green performance indicators} & 2012 \\ 
        \cite{65_Kocak2019_UtilityModel} & Kocak and Alptekin. \textit{A utility model for designing environmentally sustainable software} & 2019 \\ 
        \rowcolor{rowgray}
        \cite{57_Lago2019_DecisionMaps} & Lago. \textit{Architecture design decision maps for software sustainability} & 2019 \\ 
        \cite{11_Lago2011_SOSE} & Lago and Jansen. \textit{Creating environmental awareness in service oriented software engineering} & 2011 \\ 
        \rowcolor{rowgray}
        \cite{44_Lami2012_SoftwareMeasurement} & Lami and Buglione. \textit{Measuring software sustainability from a process-centric perspective} & 2012 \\ 
        \cite{06_Lami2014_MeasurementFramework} & Lami et al. \textit{An ISO/IEC 33000-compliant measurement framework for software process sustainability assessment} & 2014 \\ 
        \rowcolor{rowgray}
        \cite{02_Lami2013_SustainabilityIndicators} & Lami et al. \textit{A methodology to derive sustainability indicators for software development projects} & 2013 \\
        \cite{59_Lasla2022_GreenPoWAE} & Lasla et al. \textit{Green-PoW: an energy-efficient blockchain proof-of-work consensus algorithm} & 2022 \\ 
        \rowcolor{rowgray}
        \cite{58_Mahmoud2013_GreenModel} & Mahmoud and Ahmad. \textit{A green model for sustainable software engineering} & 2013 \\ 
        \cite{19_Mancebo2021_FEETINGS} & Mancebo et al. \textit{FEETINGS: Framework for energy efficiency testing to improve environmental goals of the software} & 2021 \\ 
        \rowcolor{rowgray}
        \cite{08_Mehra2023_AssessRefactoring} & Mehra et al. \textit{Assessing the impact of refactoring energy-inefficient code patterns on software sustainability: an industry case study} & 2023 \\
        \cite{38_Sharma2022_GreenQuotient} & Mehra et al. \textit{Towards a green quotient for software projects} & 2022 \\ 
        \rowcolor{rowgray}
        \cite{56_Mohankumar2016_GSDLCM} & Mohankumar and Kumar. \textit{Green based software development life cycle model for software engineering} & 2016 \\ 
        \cite{05_Moshnyaga2013_LCA} & Moshnyaga. \textit{An assessment of software lifecycle energy} & 2013 \\
        \rowcolor{rowgray}
        \cite{09_Moshnyaga2013_AssessLContribution} & Moshnyaga. \textit{Assessment of software lifecycle energy and its contribution to green house gas emissions} & 2013 \\ 
        \cite{29_Moshnyaga2013_AssessLC} & Moshnyaga. \textit{Lifecycle energy assessment of mobile applications} & 2013 \\ 
        \rowcolor{rowgray}
        \cite{45_Naumann2011_GREENSOFT} & Naumann et al. \textit{The GREENSOFT model: a reference model for green and sustainable software and its engineering} & 2011 \\ 
        \cite{60_Naumann2015_QualityModels} & Naumann et al. \textit{Sustainable software engineering: process and quality models, life cycle, and social aspects} & 2015 \\ 
        \rowcolor{rowgray}
        \cite{04_Noureddine2012_GREENS} & Noureddine et al. \textit{A preliminary study of the impact of software engineering on GreenIT} & 2012 \\
        \cite{12_Pa2017_GreenDesignMeasurement} & Pa et al. \textit{Dashboard system for measuring green software design} & 2021 \\ 
        \rowcolor{rowgray}
        \cite{14_Pan2022_CNNDecomposition} & Pan and Rajan. \textit{Decomposing convolutional neural networks into reusable and replaceable modules} & 2022 \\ 
        \cite{53_Patterson2022_MLCO2footprint} & Patterson et al. \textit{The carbon footprint of machine learning will plateau, then shrink} & 2022 \\ 
        \rowcolor{rowgray}
        \cite{63_Penzenstadler2013_GenericModel} & Penzenstadler and Femmer. \textit{A generic model for sustainability with process-- and product-specific instances} & 2013 \\ 
        \cite{10_Ponsard2018_CaseStudy} & Ponsard et al. \textit{Building sustainable software for sustainable systems: case study of a shared pick-up and delivery service} & 2018 \\
        \rowcolor{rowgray}
        \cite{22_Radersma2022_GreenEvaluation} & Radersma. \textit{Green coding: reduce your carbon footprint} & 2022 \\ 
        \cite{35_Raisian2021_MeasurementStructure} & Raisian et al. \textit{The green software measurement structure based on sustainability perspective} & 2021 \\ 
        \rowcolor{rowgray}
        \cite{47_Sharma2015_GreenSDLC} & Sharma et al. \textit{Energy efficient software development life cycle -- an approach towards smart computing} & 2015 \\ 
        \cite{55_Shenoy2011_GreenDevelopmentModel} & Shenoy et al. \textit{Green software development model: an approach towards sustainable software development} & 2011 \\ 
        \rowcolor{rowgray}
        \cite{23_Siegmund2022_GreenConfiguration} & Siegmund et al. \textit{Green configuration: can artificial intelligence help reduce energy consumption of configurable software systems?} & 2022 \\ 
        \cite{20_Sikanda2023_GreenAIQuotient} & Sikand et al. \textit{Green AI quotient: assessing greenness of AI-based software and the way forward} & 2023 \\ 
        \rowcolor{rowgray}
        \cite{42_Simon2023_ImpactSLC} & Simon et al. \textit{Uncovering the environmental impact of software life cycle} & 2023 \\ 
        \cite{37_Tee2014_GreenKnowledge} & Tee et al. \textit{Toward developing green software development model in managing knowledge of IT practitioners for sustaining future generation} & 2014 \\ 
        \rowcolor{rowgray}
        \cite{43_Tee2014_webKM} & Tee et al. \textit{Web-based knowledge management model for managing and sharing green knowledge of software development in community of practice} & 2014 \\ 
        \cite{27_Wedyan2023_Testing} & Wedyan et al. \textit{Integration and unit testing of software energy consumption} & 2023 \\ 
        \rowcolor{rowgray}
        \cite{40_Wei2023_GreenCodeGeneration} & Wei et al. \textit{Towards greener yet powerful code generation via quantization: an empirical study} & 2023 \\ 
        \cite{41_Zhang2023_NetAI} & Zhang et al. \textit{Toward net-zero carbon emission in network AI for 6G and beyond} & 2023 \\
        \hline    
    \end{tabular}}
